Efficient, Direct, and Restricted Black-Box Graph Evasion Attacks to Any-Layer Graph Neural Networks via Influence Function

Graph neural network (GNN), the mainstream method to learn on graph data, is vulnerable to graph evasion attacks, where an attacker slightly perturbing the graph structure can fool trained GNN models. Existing work has at least one of the following drawbacks: 1) limited to directly attack two-layer GNNs; 2) inefficient; and 3) impractical, as they need to know full or part of GNN model parameters. We address the above drawbacks and propose an influence-based \emph{efficient, direct, and restricted black-box} evasion attack to \emph{any-layer} GNNs. Specifically, we first introduce two influence functions, i.e., feature-label influence and label influence, that are defined on GNNs and label propagation (LP), respectively. Then we observe that GNNs and LP are strongly connected in terms of our defined influences. Based on this, we can then reformulate the evasion attack to GNNs as calculating label influence on LP, which is \emph{inherently} applicable to any-layer GNNs, while no need to know information about the internal GNN model. Finally, we propose an efficient algorithm to calculate label influence. Experimental results on various graph datasets show that, compared to state-of-the-art white-box attacks, our attack can achieve comparable attack performance, but has a 5-50x speedup when attacking two-layer GNNs. Moreover, our attack is effective to attack multi-layer GNNs\footnote{Source code and full version is in the link: \url{https://github.com/ventr1c/InfAttack}}.

==> simplify.tex <==
\section{simplify}

\noindent We take SGC model as the Attacked model, SGC model's equation: 
\begin{equation}
    f = (\tilde{D}^{-\frac{1}{2}}\tilde{A}\tilde{D}^{-\frac{1}{2}})^2XW
\end{equation}

\noindent The objective function of our attack is as follows:
\begin{equation}
    \max_{A'}\left \{ f(A',X)_{v,c}-f(A',X)_{v,y_v} \right \}
    \quad s.t. \left \| A'-A \right \| \leqslant 2\epsilon,
\end{equation}

\noindent If we focus on the target node $v$ itself, after $k$ layers propagation, we update our objective function as follows:
\begin{equation}
\label{obj_func}
    \max_{{N_v^{(1)}}'}([h_v^{(k)}]_c - [h_v^{(k)}]_{y_v}),\ s.t.,\ \left \| N_v^{(1)}-{N_v^{(1)}}' \right \| \leqslant 2\epsilon.
\end{equation}

\noindent The feature embedding of the target node $v$ has several expressions as follows:
\begin{equation}
\begin{aligned}
\label{h_v_k}
    h_v^{(k)} = \sum_{u\in IN}\sum_{p=1}^{\varPsi}{\prod_{l=k}^1{a_{v^{(l)},v^{(l-1)}}\cdot W_l\cdot h_u^{(0)}}}, \\
\end{aligned}
\end{equation}
% h_v^{(k)} 写完整
where the influential nodes set $IN=(N_v^{(1)}, N_v^{(2)},...,N_v^{(k)})$, $N_v^{(k)}$ denotes the $k$-order neighbor of the node $v$, and $\varPsi$ is the total number of paths $v_p^k,v_p^{k-1},\cdots,v_p^{1},v_p^{0}$ of length k+1 from node $v$ to the $k$ order neighbor node $u$. $a_{v^{(l)},v^{(l-1)}}$ is the normalized of edge $(v^{l}, v^{(l-1)})$, and $a_{v^{(l)},v^{(l-1)}} = deg(v^{(l)})^{-\frac{1}{2}}deg(v^{(l-1)})^{-\frac{1}{2}}$. For any path $p$, $v_p^k$ is node $v$ and $v_p^0$ is node $u$. For $l=1,\cdots,k-1$, $v_p^{l-1}\in N_{v_p}^{(l)} $.

For the node aggregation-based GNN, we know the more $c$-labeled nodes in the immediate neighbors of node $v$, the higher probability of the node $v$ classified into $c$-label. But how to evaluate the number of $c$-labeled nodes in the $IN$ nodes for the target node $v$, because nodes in different neighborhoods have different effects and a node may belong to different neighbors at the same time. So we can't use the number of c-labeled nodes to evaluate the influence to the node $v$. Inspired by JK-nets paper, the feature influence of node $u$ on the node $v$ after $k$ layers propagation as follows:
\begin{equation}
\begin{aligned}
\label{feature_influence}
    I_f(v,u;k) & = {e^T[\frac{\partial h_v^{(k)}}{\partial h_u^{(0)}}]e } / { (\sum_{v_i \in IN}e^T[\frac{\partial h_v^{(k)}}{\partial h_{v_i}^{(0)}}]e)}\\
\end{aligned}
\end{equation}

\noindent According to the chain rule, we have the derivative $\frac{\partial h_v^{(k)}}{\partial h_u^{(0)}}$ as follows:
\begin{equation}
\begin{aligned}
\label{derivate_h_v_k}
    \frac{\partial h_v^{(k)}}{\partial h_u^{(0)}} 
    &= \sum_{p=1}^{\varPsi}{\prod_{l=k}^1{a_{v^{(l)},v^{(l-1)}}\cdot W_l}} \\
    &= {\prod_{l=1}^{k}W_l} \cdot \sum_{p=1}^{\varPsi}\prod_{l=k}^1{a_{v^{(l)},v^{(l-1)}}} \\
\end{aligned}
\end{equation}

\noindent In Equation (\ref{feature_influence}), the value of the denominator can be ignored because it is a constant, we bring Equation (\ref{derivate_h_v_k}) into Equation (\ref{feature_influence}):
\begin{equation}
\begin{aligned}
    I_f(v,u;k) 
    & = {e^T[\frac{\partial h_v^{(k)}}{\partial h_u^{(0)}}]e} \\
    & = {e^T[{\prod_{l=1}^{k}W_l} \cdot  \sum_{p=1}^{\varPsi}\prod_{l=k}^1{a_{v^{(l)},v^{(l-1)}}}]e} \\
    & = {e^T[{\prod_{l=1}^{k}W_l}]e \cdot  \sum_{p=1}^{\varPsi}\prod_{l=k}^1{a_{v^{(l)},v^{(l-1)}}}} \\
    & = C \cdot \sum_{p=1}^{\varPsi}\prod_{l=k}^1{a_{v^{(l)},v^{(l-1)}}} \\
\end{aligned}
\end{equation}
where $C$ is the constant for the trained SGC model, The latter part is the probability of random walk from node $u$ to node $v$. So we can use it as an evaluation indicator, but we need to distinguish the impact of nodes with different labels on node $v$, below we give the assumption of feature independence:

\noindent \textbf{Hypothesis 1: (Strong feature independence)} The features of different types of nodes are independent of each other during the propagation process and are not affected by each other.

So we want the node $v$ label to be $c$, we only need to consider the feature influence of node $u$ with $c$-labeled, if the node $v$ label is $y_v$, we only consider the feature influence of node u with $y_v$ label. We update (\ref{obj_func}) equation as follows:
\begin{equation}
\begin{aligned}
\label{hyp1}
    & \max_{{N_v^{(1)}}'}(\sum_{\substack{u\in IN \\ y_u=c}}| I_f(v,u;k) |
    -\sum_{\substack{z\in IN \\ y_z=y_v}}| I_f(v,z;k) |) \\
    & \Leftrightarrow  \max_{{N_v^{(1)}}'}(\sum_{\substack{u\in IN \\ y_u=c}}\sum_{P_k^{u\rightarrow v}}
    \prod_{l=k}^{1}a_{v^{(l)},v^{(l-1)}} - \sum_{\substack{z\in IN \\ y_u=y_v}}
    \sum_{P_k^{z\rightarrow v}} \prod_{l=k}^{1}a_{v^{(l)},v^{(l-1)}}) \\
    & s.t. \left \| N_v^{(1)}-{N_v^{(1)}}' \right \| \leqslant 2\epsilon
\end{aligned}
\end{equation}

If we directly calculate the term $\sum_{P_k^{u\rightarrow v}}
\prod_{l=k}^{1}a_{v^{(l)},v^{(l-1)}}$, it's more complicated. So we introduce the LPA model to transform the calculation process, LPA model equation as follows:
\begin{equation}
    Y^{(k+1)}=\tilde{D}^{-\frac{1}{2}}\tilde{A}\tilde{D}^{-\frac{1}{2}}Y^{(k)}; \quad \quad
    y^{(k+1)}_i = y^{(0)}_i, \forall i \leqslant m
\end{equation}

\noindent According to the GCN-LPA paper, we have the label influence as follows:
\begin{equation}
\begin{aligned}
\label{label_influence}
    I_l(v,u;k) 
    & = \frac{\partial y_v^{(k)}}{\partial y_u^{(0)}} \\
    & = \sum_{j=d}^k \sum_{U_j^{u\rightarrow v}} \prod_{i=j}^{1}a_{v^{(i)},v^{(i-1)}} \\
\end{aligned}
\end{equation}
where $d$ is the shortest path from node $v$ to node $u$, $U_j^{u\rightarrow v}$ is a path$[v^{(k)},v^{(k-1)},...,v^{(0)}]$ of length j from node v to node u without going through the label node. We find the expression between the feature influence and the label influence is different, because the LPA model have reset the initial label in every propagation. So we readjusted the LPA model and named it as FLP model:
\begin{equation}
    Y^{(k+1)}=\tilde{D}^{-\frac{1}{2}}\tilde{A}\tilde{D}^{-\frac{1}{2}}Y^{(k)}, \quad Y^{(0)} = Y.
\end{equation}
We updated Equation (\ref{label_influence}) according to Equation (\ref{derivate_h_v_k}):
\begin{equation}
\begin{aligned}
    I_l(v,u;k) = \sum_{p=1}^{\varPsi}{\prod_{l=k}^1{a_{v^{(l)},v^{(l-1)}}}} 
\end{aligned}
\end{equation}

Since different label dimensions in $y_v^{(\cdot )}$ do not interact with each other when running FLP model, the value of the $y_v$-th dimension in $y_v^{(\cdot )}$(denoted by $y_v^{(\cdot )}[y_v]$) comes only from the nodes with the initial label $y_v$. It is clear that 
\begin{equation}
\begin{aligned}
\label{flp_out}
    y_v^{(k)}[y_v] 
    & =\sum_{\substack{u\in IN \\ y_u=y_v}} \sum_{p=1}^{\varPsi}{\prod_{l=k}^1{a_{v^{(l)},v^{(l-1)}}}} \\
    & = \sum_{\substack{z\in IN \\ y_u=y_v}}
    \sum_{P_k^{z\rightarrow v}} \prod_{l=k}^{1}a_{v^{(l)},v^{(l-1)}}) \\
\end{aligned}
\end{equation}

\noindent We take Equation \ref{flp_out} into Equation \ref{hyp1}:
\begin{equation}
\begin{aligned}
    & \max_{{N_v^{(1)}}'}(\sum_{\substack{u\in IN \\ y_u=c}}| I_f(v,u;k) |
    -\sum_{\substack{z\in IN \\ y_z=y_v}}| I_f(v,z;k) |) \\
    & \Leftrightarrow  \max_{{N_v^{(1)}}'}(y_v^{(k)}[c] - y_v^{(k)}[y_v]) \\
    & s.t. \left \| N_v^{(1)}-{N_v^{(1)}}' \right \| \leqslant 2\epsilon.
\end{aligned}
\end{equation}
Hence, we convert the problem of attacking the SGC model to attack the FLP model successfully.
